Model-Ensemble Trust-Region Policy Optimization

Model-free reinforcement learning (RL) methods are succeeding in a growing number of tasks, aided by recent advances in deep learning. However, they tend to suffer from high sample complexity, which hinders their use in real-world domains. Alternatively, model-based reinforcement learning promises to reduce sample complexity, but tends to require careful tuning and to date have succeeded mainly in restrictive domains where simple models are sufficient for learning. In this paper, we analyze the behavior of vanilla model-based reinforcement learning methods when deep neural networks are used to learn both the model and the policy, and show that the learned policy tends to exploit regions where insufficient data is available for the model to be learned, causing instability in training. To overcome this issue, we propose to use an ensemble of models to maintain the model uncertainty and regularize the learning process. We further show that the use of likelihood ratio derivatives yields much more stable learning than backpropagation through time. Altogether, our approach Model-Ensemble Trust-Region Policy Optimization (ME-TRPO) significantly reduces the sample complexity compared to model-free deep RL methods on challenging continuous control benchmark tasks.

==> illustration.tex <==
\section{A Motivating Example}
\TODO{figure out if we want this section.}
We motivate our approach by illustrating the fundamental difficulty in model based optimization with expressive neural networks. Consider optimizing the function $f(x)$ shown in the black line in Figure \ref{fig:illustration}. The function $f$ has a global minimum at $x=1.7$, and a local minimum at $x=4.4$, We initialize our solution to $x_0 = 2.5$, which belongs to the basin of the global minimum, and sample function values normally distributed around $x_0$, marked by red circles in the figure. To these samples we fit a neural network $\tilde{f}(x)$, as shown by the blue line in Figure \ref{fig:illustration}. As expected, the neural network fit is accurate in the vicinity of $x_0$. However, the global minimum of $\tilde{f}$ is around $4$, which belongs to the basin of the suboptimal local minimum for $f$. Thus, naively optimizing $\tilde{f}$ will lead to a degradation in the true objective $f$. This issue could be mitigated by constraining the optimization to the vicinity of $x_0$. The validation model approach explored in this work provides a simple means to implicitly enforce such a constraint.  
\begin{figure}[h]
\caption{An illustrative example}\label{fig:illustration}
\centering
\includegraphics[width=0.4\textwidth]{nn_fit}
\end{figure}

%%PA: I like the gist of this section a lot, esp. because it's so simple.  That said, the current figure doesn't work well;  Here is why: (i) it's distracting to have multiple local optima in the original function, that's not really what we are worried about; (ii) running gradient descent on the learning neural net will actually take you to where you want to be, so it does *not* illustrate how neural-net model-based optimization fails (b/c it actually succeeds!);   --> what we 'd want is ideally an original function with only 1 local optimum, and most importantly we want the fitted neural net leading the optimization algorithm to go in the wrong direction  
